Unstable Unlearning: The Hidden Risk of Concept Resurgence in Diffusion Models

Text-to-image diffusion models rely on massive, web-scale datasets. Training them from scratch is computationally expensive, and as a result, developers often prefer to make incremental updates to existing models. These updates often compose fine-tuning steps (to learn new concepts or improve model performance) with "unlearning" steps (to "forget" existing concepts, such as copyrighted works or explicit content). In this work, we demonstrate a critical and previously unknown vulnerability that arises in this paradigm: even under benign, non-adversarial conditions, fine-tuning a text-to-image diffusion model on seemingly unrelated images can cause it to "relearn" concepts that were previously "unlearned." We comprehensively investigate the causes and scope of this phenomenon, which we term concept resurgence, by performing a series of experiments which compose "concept unlearning" with subsequent fine-tuning of Stable Diffusion v1.4 and Stable Diffusion v2.1. Our findings underscore the fragility of composing incremental model updates, and raise serious new concerns about current approaches to ensuring the safety and alignment of text-to-image diffusion models.

==> figures/results.tex <==

\begin{table}[htbp]
\caption{Unlearning performance before and after fine-tuning for Stable Diffusion v1.4. Each metric is task-specific, and evaluates the ability to generate the unwanted concept (lower is better; see \Cref{sec:warmup} for details). Results for SDD on unsafe content are excluded as first-stage unlearning compromises the model's ability to generate \emph{any} images, including retained concepts.}
\label{tab:performance}
\resizebox{\textwidth}{!}{ % Resize to fit the width of the page
\begin{tabular}[t]{l l r r}
\toprule
 &  & Before FT & After FT \\
Task & Method &  &  \\
\midrule
\multirow[t]{4}{*}{\textbf{celebrity}} & \textbf{ESD} & 0.144 $\pm$ 0.011 & 0.950 $\pm$ 0.007 \\
\textbf{} & \textbf{MACE} & 0.042 $\pm$ 0.004 & 0.391 $\pm$ 0.043 \\
\textbf{} & \textbf{SDD} & 0.556 $\pm$ 0.203 & 0.965 $\pm$ 0.008 \\
\textbf{} & \textbf{UCE} & 0.001 $\pm$ 0.001 & 0.004 $\pm$ 0.002 \\
\textbf{} & \textbf{EraseDiff} & 0.000 $\pm$ 0.000 & 0.693 $\pm$ 0.019 \\
\textbf{} & \textbf{SHS} & 0.075 $\pm$ 0.019 & 0.893 $\pm$ 0.054 \\
\textbf{} & \textbf{SalUn} & 0.363 $\pm$ 0.082 & 0.939 $\pm$ 0.056 \\
\cline{1-4}
\multirow[t]{4}{*}{\textbf{copyright}} & \textbf{ESD} & 0.000 $\pm$ 0.000 & 0.100 $\pm$ 0.067 \\
\textbf{} & \textbf{MACE} & 0.100 $\pm$ 0.100 & 0.267 $\pm$ 0.167 \\
\textbf{} & \textbf{SDD} & 0.000 $\pm$ 0.000 & 0.100 $\pm$ 0.033 \\
\textbf{} & \textbf{UCE} & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 \\
\textbf{} & \textbf{EraseDiff} & 0.000 $\pm$ 0.000 & 0.367 $\pm$ 0.033 \\
\textbf{} & \textbf{SHS} & 0.000 $\pm$ 0.000 & 0.133 $\pm$ 0.033 \\
\textbf{} & \textbf{SalUn} & 0.000 $\pm$ 0.033 & 0.100 $\pm$ 0.067 \\
\cline{1-4}
\multirow[t]{4}{*}{\textbf{object}} & \textbf{ESD} & 0.192 $\pm$ 0.032 & 0.990 $\pm$ 0.008 \\
\textbf{} & \textbf{MACE} & 0.045 $\pm$ 0.005 & 0.033 $\pm$ 0.003 \\
\textbf{} & \textbf{SDD} & 0.000 $\pm$ 0.007 & 0.355 $\pm$ 0.073 \\
\textbf{} & \textbf{UCE} & 0.023 $\pm$ 0.000 & 0.030 $\pm$ 0.020 \\
\textbf{} & \textbf{EraseDiff} & 0.002 $\pm$ 0.002 & 0.995 $\pm$ 0.001 \\
\textbf{} & \textbf{SHS} & 0.399 $\pm$ 0.274 & 0.999 $\pm$ 0.001 \\
\textbf{} & \textbf{SalUn} & 0.831 $\pm$ 0.531 & 0.913 $\pm$ 0.065 \\
\cline{1-4}
\multirow[t]{4}{*}{\textbf{unsafe}} & \textbf{ESD} & 0.547 $\pm$ 0.073 & 0.840 $\pm$ 0.024 \\
\textbf{} & \textbf{MACE} & 0.275 $\pm$ 0.058 & 0.319 $\pm$ 0.042 \\
\textbf{} & \textbf{SDD} & N/A & N/A \\
\textbf{} & \textbf{UCE} & 0.649 $\pm$ 0.010 & 0.670 $\pm$ 0.013 \\
\textbf{} & \textbf{EraseDiff} & 0.317 $\pm$ 0.181 & 0.876 $\pm$ 0.017 \\
\textbf{} & \textbf{SHS} & 0.403 $\pm$ 0.058 & 0.848 $\pm$ 0.024 \\
\textbf{} & \textbf{SalUn} & 0.840 $\pm$ 0.217 & 0.872 $\pm$ 0.008 \\
\cline{1-4}
\bottomrule
\end{tabular}
} % End resizebox
\end{table}


==> figures/results_SD21_iclr.tex <==
\begin{table}[htbp]
\caption{Unlearning performance before and after fine-tuning for Stable Diffusion v2.1. Each metric is task-specific, and evaluates the ability to generate the unwanted concept (lower is better; see \Cref{sec:warmup} for details). Results for SDD on unsafe content are excluded as first-stage unlearning compromises the model's ability to generate \emph{any} images, including retained concepts.}
\label{tab:performance_sd21}
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}[t]{l l r r}
\toprule
 &  & Before FT & After FT \\
Task & Algorithm &  &  \\
\midrule
\multirow[t]{3}{*}{\textbf{celebrity}} & \textbf{ESD} & 0.291 $\pm$ 0.095 & 0.929 $\pm$ 0.011 \\
\textbf{} & \textbf{SDD} & 0.804 $\pm$ 0.087 & 0.934 $\pm$ 0.023 \\
\textbf{} & \textbf{UCE} & 0.002 $\pm$ 0.000 & 0.004 $\pm$ 0.001 \\
\cline{1-4}
\multirow[t]{3}{*}{\textbf{copyright}} & \textbf{ESD} & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.033 \\
\textbf{} & \textbf{SDD} & 0.000 $\pm$ 0.000 & 0.167 $\pm$ 0.100 \\
\textbf{} & \textbf{UCE} & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 \\
\cline{1-4}
\multirow[t]{3}{*}{\textbf{unsafe}} & \textbf{ESD} & 0.155 $\pm$ 0.023 & 0.780 $\pm$ 0.013 \\
\textbf{} & \textbf{SDD} & N/A & N/A \\
\textbf{} & \textbf{UCE} & 0.652 $\pm$ 0.000 & 0.715 $\pm$ 0.021 \\
\cline{1-4}
\bottomrule
\end{tabular}%
}
\end{table}



==> figures/results_SD21_old.tex <==
\begin{table}[htbp]
\caption{Performance metrics before and after fine-tuning}
\label{tab:performance}
\begin{tabular}{l l r r}
\toprule
 &  & After Finetuning & Before Finetuning \\
task & algo &  &  \\
\midrule
\multirow[t]{3}{*}{\textbf{celebrity}} & \textbf{ESD} & 0.929 (0.918-0.930) & 0.291 (0.196-0.292) \\
\textbf{} & \textbf{SDD} & 0.934 (0.934-0.958) & 0.804 (0.803-0.891) \\
\textbf{} & \textbf{UCE} & 0.004 (0.004-0.005) & 0.002 (0.002-0.002) \\
\cline{1-4}
\multirow[t]{3}{*}{\textbf{copyright}} & \textbf{ESD} & 0.000 (0.000-0.033) & 0.000 (0.000-0.000) \\
\textbf{} & \textbf{SDD} & 0.167 (0.133-0.267) & 0.000 (0.000-0.000) \\
\textbf{} & \textbf{UCE} & 0.000 (0.000-0.000) & 0.000 (0.000-0.000) \\
\cline{1-4}
\multirow[t]{3}{*}{\textbf{unsafe_content}} & \textbf{ESD} & 0.780 (0.767-0.783) & 0.155 (0.146-0.177) \\
\textbf{} & \textbf{SDD} & N/A & N/A \\
\textbf{} & \textbf{UCE} & 0.715 (0.694-0.736) & 0.517 \\
\cline{1-4}
\bottomrule
\end{tabular}
\end{table}


==> figures/results_iclr.tex <==
% \begin{table}[htbp]
% \caption{Unlearning performance before and after fine-tuning for Stable Diffusion v1.4. Each metric is task-specific, and evaluates the ability to generate the unwanted concept (lower is better; see \Cref{sec:warmup} for details). Results for SDD on unsafe content are excluded as first-stage unlearning compromises the model's ability to generate \emph{any} images, including retained concepts.}
% \label{tab:performance}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l c c c c c c c c}
% \toprule
%  & \multicolumn{2}{c}{\textbf{Celebrity}} & \multicolumn{2}{c}{\textbf{Copyright}} & \multicolumn{2}{c}{\textbf{Object}} & \multicolumn{2}{c}{\textbf{Unsafe}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
% \textbf{Method} & Before FT & After FT & Before FT & After FT & Before FT & After FT & Before FT & After FT \\
% \midrule
% \textbf{ESD} & 0.144 $\pm$ 0.011 & 0.950 $\pm$ 0.007 & 0.000 $\pm$ 0.000 & 0.100 $\pm$ 0.067 & 0.192 $\pm$ 0.032 & 0.990 $\pm$ 0.008 & 0.547 $\pm$ 0.073 & 0.840 $\pm$ 0.024 \\
% \textbf{MACE} & 0.042 $\pm$ 0.004 & 0.391 $\pm$ 0.043 & 0.100 $\pm$ 0.100 & 0.267 $\pm$ 0.167 & 0.045 $\pm$ 0.005 & 0.033 $\pm$ 0.003 & 0.275 $\pm$ 0.058 & 0.319 $\pm$ 0.042 \\
% \textbf{SDD} & 0.556 $\pm$ 0.203 & 0.965 $\pm$ 0.008 & 0.000 $\pm$ 0.000 & 0.100 $\pm$ 0.033 & 0.000 $\pm$ 0.007 & 0.355 $\pm$ 0.073 & N/A & N/A \\
% \textbf{UCE} & 0.001 $\pm$ 0.001 & 0.004 $\pm$ 0.002 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 & 0.023 $\pm$ 0.000 & 0.030 $\pm$ 0.020 & 0.649 $\pm$ 0.010 & 0.670 $\pm$ 0.013 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[t]
\caption{Unlearning performance before and after fine-tuning for Stable Diffusion v1.4 (Part 1). Each metric is task-specific, and evaluates the ability to generate the unwanted concept (lower is better; see \Cref{sec:warmup} for details).}
\label{tab:performance}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{l c c c c}
\toprule
 & \multicolumn{2}{c}{\textbf{Celebrity}} & \multicolumn{2}{c}{\textbf{Copyright}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Method} & Before FT & After FT & Before FT & After FT \\
\midrule
\textbf{ESD} & 0.144 $\pm$ 0.011 & 0.950 $\pm$ 0.007 & 0.000 $\pm$ 0.000 & 0.100 $\pm$ 0.067 \\
\textbf{MACE} & 0.042 $\pm$ 0.004 & 0.391 $\pm$ 0.043 & 0.100 $\pm$ 0.100 & 0.267 $\pm$ 0.167 \\
\textbf{SDD} & 0.556 $\pm$ 0.203 & 0.965 $\pm$ 0.008 & 0.000 $\pm$ 0.000 & 0.100 $\pm$ 0.033 \\
\textbf{UCE} & 0.001 $\pm$ 0.001 & 0.004 $\pm$ 0.002 & 0.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[t]
\caption{Unlearning performance before and after fine-tuning for Stable Diffusion v1.4 (Part 2). Each metric is task-specific, and evaluates the ability to generate the unwanted concept (lower is better; see \Cref{sec:warmup} for details). Results for SDD on unsafe content are excluded as first-stage unlearning compromises the model's ability to generate \emph{any} images, including retained concepts.}
\label{tab:performance_2}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{l c c c c}
\toprule
 & \multicolumn{2}{c}{\textbf{Object}} & \multicolumn{2}{c}{\textbf{Unsafe}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Method} & Before FT & After FT & Before FT & After FT \\
\midrule
\textbf{ESD} & 0.192 $\pm$ 0.032 & 0.990 $\pm$ 0.008 & 0.547 $\pm$ 0.073 & 0.840 $\pm$ 0.024 \\
\textbf{MACE} & 0.045 $\pm$ 0.005 & 0.033 $\pm$ 0.003 & 0.275 $\pm$ 0.058 & 0.319 $\pm$ 0.042 \\
\textbf{SDD} & 0.000 $\pm$ 0.007 & 0.355 $\pm$ 0.073 & N/A & N/A \\
\textbf{UCE} & 0.023 $\pm$ 0.000 & 0.030 $\pm$ 0.020 & 0.649 $\pm$ 0.010 & 0.670 $\pm$ 0.013 \\
\bottomrule
\end{tabular}%
}
\end{table}

